Plotting time: On the usage of CNNs for time series classification

We present a novel approach for time series classification where we represent time series data as plot images and feed them to a simple CNN, outperforming several state-of-the-art methods. We propose a simple and highly replicable way of plotting the time series, and feed these images as input to a non-optimized shallow CNN, without any normalization or residual connections. These representations are no more than default line plots using the time series data, where the only pre-processing applied is to reduce the number of white pixels in the image. We compare our method with different state-of-the-art methods specialized in time series classification on two real-world non public datasets, as well as 98 datasets of the UCR dataset collection. The results show that our approach is very promising, achieving the best results on both real-world datasets and matching / beating the best state-of-the-art methods in six UCR datasets. We argue that, if a simple naive design like ours can obtain such good results, it is worth further exploring the capabilities of using image representation of time series data, along with more powerful CNNs, for classification and other related tasks.

==> tables/rankByDataset_bornBetweenJune21AndJuly22.tex <==
\begin{table*}[!h]
\centering
\caption{ Legenda *** }
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc}
&$1^{st}$&$2^{nd}$&$3^{rd}$\\ 
\hline
ACSF1&ResNet (0.93)&HIVE-COTE v1.0 \& STC \& WEASEL (0.92)&\\ 
Adiac&InceptionTime (0.851662404)&ResNet (0.849104859)&WEASEL (0.826086957)\\ 
ArrowHead&TS-CHIEF \& ProximityForest (0.948571429)&InceptionTime \& S-BOSS (0.937142857)\\ 
Beef&STC (1.0)&WEASEL \& RISE (0.933333333)&\\ 
BeetleFly&TS-CHIEF \& HIVE-COTE v1.0 \& ROCKET \& InceptionTime \& STC \& ResNet \& ProximityForest \& S-BOSS \& cBOSS \& BOSS \& RISE (1.0)&\\ 
BirdChicken&TS-CHIEF \& HIVE-COTE v1.0 \& ROCKET \& InceptionTime \& STC \& ResNet \& ProximityForest \& WEASEL \& S-BOSS \& cBOSS \& BOSS \& RISE \& TSF \& Catch22 (1.0)&\\ 
BME&CNN \& TS-CHIEF \& HIVE-COTE v1.0 \& ROCKET \& InceptionTime \& ResNet \& ProximityForest \& WEASEL (1.0)&\\ 
Car&InceptionTime (0.966666667)&TS-CHIEF \& HIVE-COTE v1.0 \& ROCKET \& STC \& ResNet \& S-BOSS (0.95)&\\ 
CBF&TS-CHIEF \& HIVE-COTE v1.0 \& ROCKET \& InceptionTime \& ResNet \& ProximityForest \& WEASEL \& S-BOSS \& cBOSS \& BOSS \& TSF (1.0)&\\ 
Chinatown&InceptionTime (0.988338192)&ResNet (0.985507246)&ROCKET \& STC \& TSF (0.982507289)\\ 
ChlorineConcentration&InceptionTime (0.89296875)&ResNet (0.8703125)&ROCKET (0.834635417)\\ 
CinCECGTorso&HIVE-COTE v1.0 (1.0)&WEASEL (0.999275362)&S-BOSS (0.998550725)\\ 
Coffee&CNN \& TS-CHIEF \& HIVE-COTE v1.0 \& ROCKET \& InceptionTime \& STC \& ResNet \& ProximityForest \& WEASEL \& S-BOSS \& cBOSS \& BOSS \& RISE \& TSF \& Catch22 (1.0)&\\ 
Computers&InceptionTime (0.904)&ResNet (0.892)&ROCKET (0.884)\\ 
Crop&InceptionTime (0.796785714)&HIVE-COTE v1.0 (0.773035714)&ResNet (0.772380952)\\ 
DiatomSizeReduction&InceptionTime (1.0)&ROCKET \& BOSS (0.993464052)&\\ 
DistalPhalanxOutlineAgeGroup&S-BOSS (0.90647482)&TS-CHIEF \& HIVE-COTE v1.0 \& BOSS (0.899280576)&\\ 
DistalPhalanxOutlineCorrect&ROCKET \& ProximityForest (0.869565217)&TS-CHIEF \& HIVE-COTE v1.0 (0.865942029)\\ 
DistalPhalanxTW&HIVE-COTE v1.0 \& ProximityForest \& Catch22 (0.741007194)&\\ 
Earthquakes&CNN (0.777)&ProximityForest (0.769784173)&InceptionTime \& ResNet \& Catch22 (0.762589928)\\ 
ECG200&ResNet (0.95)&ROCKET \& InceptionTime (0.94)&\\ 
ECG5000&TS-CHIEF (0.952)&WEASEL (0.951333333)&ROCKET (0.950888889)\\ 
ECGFiveDays&TS-CHIEF \& HIVE-COTE v1.0 \& ROCKET \& InceptionTime \& STC \& WEASEL \& S-BOSS \& cBOSS \& BOSS (1.0)&\\ 
ElectricDevices&ROCKET (0.904551939)&InceptionTime (0.904162884)&ResNet (0.899753599)\\ 
EthanolLevel&ResNet (0.908)&InceptionTime (0.904)&STC (0.886)\\ 
FaceAll&InceptionTime \& ResNet (0.99408284)&ROCKET (0.993491124)\\ 
FaceFour&TS-CHIEF \& HIVE-COTE v1.0 \& WEASEL \& S-BOSS \& cBOSS \& BOSS (1.0)&\\ 
FacesUCR&InceptionTime (0.985853659)&TS-CHIEF (0.983902439)&ROCKET (0.981463415)\\ 
FiftyWords&TS-CHIEF \& InceptionTime (0.865934066)&ProximityForest (0.850549451)\\ 
Fish&TS-CHIEF \& HIVE-COTE v1.0 \& cBOSS (1.0)&\\ 
FordA&WEASEL (0.976515152)&InceptionTime (0.968939394)&TS-CHIEF (0.959090909)\\ 
FreezerRegularTrain&HIVE-COTE v1.0 \& STC (1.0)&TS-CHIEF (0.999649123)\\ 
FreezerSmallTrain&HIVE-COTE v1.0 \& STC (1.0)&Catch22 (0.999649123)\\ 
GunPoint&TS-CHIEF \& HIVE-COTE v1.0 \& InceptionTime \& STC \& ResNet \& WEASEL \& S-BOSS \& cBOSS \& BOSS \& RISE (1.0)&\\ 
GunPointAgeSpan&TS-CHIEF \& HIVE-COTE v1.0 \& ROCKET \& ResNet \& ProximityForest \& WEASEL \& S-BOSS \& cBOSS \& BOSS (1.0)&\\ 
GunPointMaleVersusFemale&TS-CHIEF \& HIVE-COTE v1.0 \& ROCKET \& InceptionTime \& ResNet \& ProximityForest \& WEASEL \& S-BOSS \& cBOSS \& BOSS \& RISE \& TSF (1.0)&\\ 
GunPointOldVersusYoung&TS-CHIEF \& HIVE-COTE v1.0 \& ROCKET \& InceptionTime \& ResNet \& ProximityForest \& WEASEL \& S-BOSS \& cBOSS \& BOSS \& RISE \& TSF \& Catch22 (1.0)&\\ 
Ham&ProximityForest (1.0)&ROCKET (0.996825397)&Catch22 (0.984126984)\\ 
Haptics&HIVE-COTE v1.0 (0.948648649)&ResNet (0.935135135)&ROCKET (0.923809524)\\ 
Herring&Catch22 (0.905405405)&S-BOSS (0.734375)&InceptionTime \& STC \& BOSS (0.71875)\\ 
HouseTwenty&TS-CHIEF \& InceptionTime \& STC \& S-BOSS (0.991596639)&\\ 
InlineSkate&HIVE-COTE v1.0 (1.0)&ROCKET \& ResNet \& ProximityForest (0.991596639)&\\ 
InsectEPGRegularTrain&TS-CHIEF \& InceptionTime \& STC \& WEASEL \& S-BOSS \& cBOSS \& BOSS \& RISE \& TSF (1.0)&\\ 
InsectEPGSmallTrain&TS-CHIEF \& HIVE-COTE v1.0 \& ROCKET \& InceptionTime \& ResNet \& ProximityForest \& S-BOSS \& cBOSS \& BOSS \& TSF (1.0)&\\ 
ItalyPowerDemand&TS-CHIEF \& InceptionTime (0.972789116)&CNN (0.9708)\\ 
LargeKitchenAppliances&InceptionTime (0.973333333)&ResNet (0.971817298)&ROCKET (0.969873664)\\ 
Lightning2&ResNet (0.976)&HIVE-COTE v1.0 (0.952)&ROCKET (0.949333333)\\ 
Lightning7&Catch22 (0.925333333)&ProximityForest (0.918032787)&ResNet (0.901639344)\\ 
Mallat&TS-CHIEF (0.997867804)&WEASEL (0.985074627)&InceptionTime (0.980383795)\\ 
Meat&TS-CHIEF \& InceptionTime \& STC \& WEASEL \& S-BOSS \& cBOSS \& BOSS \& RISE \& TSF (1.0)&\\ 
MedicalImages&HIVE-COTE v1.0 \& ROCKET \& ResNet \& ProximityForest (1.0)&\\ 
MiddlePhalanxOutlineAgeGroup&Catch22 (0.983333333)&ROCKET (0.828947368)&ResNet (0.823684211)\\ 
MiddlePhalanxOutlineCorrect&STC (0.869415808)&InceptionTime (0.865979381)&WEASEL (0.855670103)\\ 
MiddlePhalanxTW&ROCKET (0.865979381)&ProximityForest (0.862542955)&ResNet (0.855670103)\\ 
MixedShapesRegularTrain&TS-CHIEF (0.981030928)&InceptionTime \& WEASEL (0.975257732)&\\ 
MixedShapesSmallTrain&ResNet (0.978969072)&HIVE-COTE v1.0 (0.976907216)&ROCKET (0.974845361)\\ 
MoteStrain&TS-CHIEF (0.96884984)&HIVE-COTE v1.0 (0.966185567)&WEASEL (0.956070288)\\ 
OliveOil&STC \& RISE \& TSF (1.0)&\\ 
OSULeaf&ROCKET \& ProximityForest (1.0)&TS-CHIEF \& S-BOSS (0.995867769)\\ 
PhalangesOutlinesCorrect&HIVE-COTE v1.0 (0.962340967)&ROCKET (0.958677686)&ResNet (0.956234097)\\ 
Phoneme&HIVE-COTE v1.0 \& ResNet (0.966666667)&Catch22 (0.883969466)\\ 
PigAirwayPressure&STC (0.995192308)&HIVE-COTE v1.0 \& ResNet (0.987603306)&\\ 
PigArtPressure&S-BOSS (1.0)&TS-CHIEF \& InceptionTime \& cBOSS \& BOSS (0.995192308)&\\ 
PigCVP&TS-CHIEF (0.985576923)&S-BOSS (0.980769231)&cBOSS \& BOSS (0.975961538)\\ 
Plane&CNN \& TS-CHIEF \& InceptionTime \& STC \& WEASEL \& S-BOSS \& cBOSS \& BOSS \& RISE \& TSF (1.0)&\\ 
ProximalPhalanxOutlineAgeGroup&ProximityForest (1.0)&ROCKET (0.988888889)&HIVE-COTE v1.0 (0.975961538)\\ 
ProximalPhalanxOutlineCorrect&HIVE-COTE v1.0 \& ResNet (1.0)&InceptionTime (0.93814433)\\ 
ProximalPhalanxTW&HIVE-COTE v1.0 \& Catch22 (1.0)&ResNet (0.922222222)\\ 
RefrigerationDevices&Catch22 (0.938888889)&HIVE-COTE v1.0 (0.887804878)&ROCKET \& ResNet (0.848780488)\\ 
Rock&STC (0.96)&WEASEL (0.94)&ResNet (0.927835052)\\ 
ScreenType&ROCKET (0.9)&Catch22 (0.865979381)&ProximityForest (0.86)\\ 
SemgHandGenderCh2&TS-CHIEF (0.968333333)&TSF (0.965)&STC (0.958333333)\\ 
SemgHandMovementCh2&ProximityForest (0.98)&ROCKET (0.95)&HIVE-COTE v1.0 (0.94)\\ 
SemgHandSubjectCh2&TSF (0.953333333)&TS-CHIEF (0.951111111)&STC (0.937777778)\\ 
ShapeletSim&TS-CHIEF \& STC \& WEASEL \& S-BOSS \& cBOSS \& BOSS (1.0)&\\ 
ShapesAll&ROCKET (1.0)&InceptionTime (0.96)&TS-CHIEF (0.958333333)\\ 
SmallKitchenAppliances&HIVE-COTE v1.0 (0.968888889)&ROCKET (0.941666667)&ProximityForest (0.911666667)\\ 
SmoothSubspace&CNN \& TS-CHIEF \& HIVE-COTE v1.0 \& TSF (1.0)&\\ 
SonyAIBORobotSurface1&ProximityForest \& Catch22 (1.0)&ROCKET (0.993333333)\\ 
SonyAIBORobotSurface2&ROCKET (0.981697171)&InceptionTime (0.974816369)&ProximityForest (0.965058236)\\ 
StarLightCurves&HIVE-COTE v1.0 \& ResNet (1.0)&TS-CHIEF (0.98348713)\\ 
Strawberry&WEASEL (0.991891892)&TS-CHIEF \& InceptionTime \& S-BOSS \& cBOSS \& BOSS \& TSF (0.989189189)&\\ 
SwedishLeaf&ROCKET \& ProximityForest (0.991891892)&ResNet (0.989506821)\\ 
Symbols&TS-CHIEF (0.987939698)&InceptionTime (0.985929648)&HIVE-COTE v1.0 (0.981787275)\\ 
SyntheticControl&TS-CHIEF \& InceptionTime \& STC \& TSF (1.0)&\\ 
ToeSegmentation1&ROCKET \& ProximityForest (1.0)&WEASEL \& S-BOSS \& cBOSS (0.986842105)\\ 
ToeSegmentation2&TS-CHIEF \& InceptionTime (0.992307692)&cBOSS \& BOSS (0.984615385)\\ 
Trace&CNN \& TS-CHIEF \& HIVE-COTE v1.0 \& InceptionTime \& STC \& ResNet \& WEASEL \& S-BOSS \& cBOSS \& BOSS \& RISE \& TSF (1.0)&\\ 
TwoLeadECG&ROCKET \& STC \& ProximityForest \& WEASEL \& cBOSS \& BOSS (1.0)&\\ 
TwoPatterns&TS-CHIEF \& ROCKET \& InceptionTime (1.0)&\\ 
UMD&TS-CHIEF \& HIVE-COTE v1.0 \& ROCKET \& InceptionTime \& ResNet \& ProximityForest (1.0)&\\ 
UWaveGestureLibraryAll&HIVE-COTE v1.0 \& ROCKET \& ResNet \& Catch22 (1.0)&\\ 
Wafer&STC \& WEASEL \& cBOSS (1.0)&\\ 
Wine&TS-CHIEF \& ROCKET \& WEASEL \& S-BOSS \& BOSS \& RISE (1.0)&\\ 
WordSynonyms&ROCKET \& ProximityForest (1.0)&TS-CHIEF (0.827586207)\\ 
Worms&HIVE-COTE v1.0 \& ResNet (1.0)&STC \& WEASEL (0.883116883)\\ 
WormsTwoClass&HIVE-COTE v1.0 \& ResNet (1.0)&Catch22 (0.999026606)\\ 
Yoga&cBOSS (0.937333333)&InceptionTime (0.933666667)&HIVE-COTE v1.0 (0.931)\\ 
\end{tabular}
}
\label{ Label *** }
\end{table*}






==> tables/rankByDataset_short.tex <==
\begin{table*}[!h]
\centering
\caption{ Legenda *** }
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc}
&$1^{st}$&$2^{nd}$&$3^{rd}$\\ 
\hline
ACSF1&ResNet (0.93)&HIVE-COTE v1.0 \& STC \& WEASEL (0.92)&\\ 
Adiac&InceptionTime (0.851662404)&ResNet (0.849104859)&WEASEL (0.826086957)\\ 
ArrowHead&TS-CHIEF \& ProximityForest (0.948571429)&InceptionTime \& S-BOSS (0.937142857)\\ 
Beef&STC (1.0)&WEASEL \& RISE (0.933333333)&\\ 
BeetleFly&Over 3 methods (1.0)&\\ 
BirdChicken&Over 3 methods (1.0)&\\ 
BME&Over 3 methods (1.0)&\\ 
Car&InceptionTime (0.966666667)&Over 3 methods (0.95)&\\ 
CBF&Over 3 methods (1.0)&\\ 
Chinatown&InceptionTime (0.988338192)&ResNet (0.985507246)&ROCKET \& STC \& TSF (0.982507289)\\ 
ChlorineConcentration&InceptionTime (0.89296875)&ResNet (0.8703125)&ROCKET (0.834635417)\\ 
CinCECGTorso&HIVE-COTE v1.0 (1.0)&WEASEL (0.999275362)&S-BOSS (0.998550725)\\ 
Coffee&Over 3 methods (1.0)&\\ 
Computers&InceptionTime (0.904)&ResNet (0.892)&ROCKET (0.884)\\ 
Crop&InceptionTime (0.796785714)&HIVE-COTE v1.0 (0.773035714)&ResNet (0.772380952)\\ 
DiatomSizeReduction&InceptionTime (1.0)&ROCKET \& BOSS (0.993464052)&\\ 
DistalPhalanxOutlineAgeGroup&S-BOSS (0.90647482)&TS-CHIEF \& HIVE-COTE v1.0 \& BOSS (0.899280576)&\\ 
DistalPhalanxOutlineCorrect&ROCKET \& ProximityForest (0.869565217)&TS-CHIEF \& HIVE-COTE v1.0 (0.865942029)\\ 
DistalPhalanxTW&HIVE-COTE v1.0 \& ProximityForest \& Catch22 (0.741007194)&\\ 
Earthquakes&CNN (0.777)&ProximityForest (0.769784173)&InceptionTime \& ResNet \& Catch22 (0.762589928)\\ 
ECG200&ResNet (0.95)&ROCKET \& InceptionTime (0.94)&\\ 
ECG5000&TS-CHIEF (0.952)&WEASEL (0.951333333)&ROCKET (0.950888889)\\ 
ECGFiveDays&Over 3 methods (1.0)&\\ 
ElectricDevices&ROCKET (0.904551939)&InceptionTime (0.904162884)&ResNet (0.899753599)\\ 
EthanolLevel&ResNet (0.908)&InceptionTime (0.904)&STC (0.886)\\ 
FaceAll&InceptionTime \& ResNet (0.99408284)&ROCKET (0.993491124)\\ 
FaceFour&Over 3 methods (1.0)&\\ 
FacesUCR&InceptionTime (0.985853659)&TS-CHIEF (0.983902439)&ROCKET (0.981463415)\\ 
FiftyWords&TS-CHIEF \& InceptionTime (0.865934066)&ProximityForest (0.850549451)\\ 
Fish&TS-CHIEF \& HIVE-COTE v1.0 \& cBOSS (1.0)&\\ 
FordA&WEASEL (0.976515152)&InceptionTime (0.968939394)&TS-CHIEF (0.959090909)\\ 
FreezerRegularTrain&HIVE-COTE v1.0 \& STC (1.0)&TS-CHIEF (0.999649123)\\ 
FreezerSmallTrain&HIVE-COTE v1.0 \& STC (1.0)&Catch22 (0.999649123)\\ 
GunPoint&Over 3 methods (1.0)&\\ 
GunPointAgeSpan&Over 3 methods (1.0)&\\ 
GunPointMaleVersusFemale&Over 3 methods (1.0)&\\ 
GunPointOldVersusYoung&Over 3 methods (1.0)&\\ 
Ham&ProximityForest (1.0)&ROCKET (0.996825397)&Catch22 (0.984126984)\\ 
Haptics&HIVE-COTE v1.0 (0.948648649)&ResNet (0.935135135)&ROCKET (0.923809524)\\ 
Herring&Catch22 (0.905405405)&S-BOSS (0.734375)&InceptionTime \& STC \& BOSS (0.71875)\\ 
HouseTwenty&Over 3 methods (0.991596639)&\\ 
InlineSkate&HIVE-COTE v1.0 (1.0)&ROCKET \& ResNet \& ProximityForest (0.991596639)&\\ 
InsectEPGRegularTrain&Over 3 methods (1.0)&\\ 
InsectEPGSmallTrain&Over 3 methods (1.0)&\\ 
ItalyPowerDemand&TS-CHIEF \& InceptionTime (0.972789116)&CNN (0.9708)\\ 
LargeKitchenAppliances&InceptionTime (0.973333333)&ResNet (0.971817298)&ROCKET (0.969873664)\\ 
Lightning2&ResNet (0.976)&HIVE-COTE v1.0 (0.952)&ROCKET (0.949333333)\\ 
Lightning7&Catch22 (0.925333333)&ProximityForest (0.918032787)&ResNet (0.901639344)\\ 
Mallat&TS-CHIEF (0.997867804)&WEASEL (0.985074627)&InceptionTime (0.980383795)\\ 
Meat&Over 3 methods (1.0)&\\ 
MedicalImages&Over 3 methods (1.0)&\\ 
MiddlePhalanxOutlineAgeGroup&Catch22 (0.983333333)&ROCKET (0.828947368)&ResNet (0.823684211)\\ 
MiddlePhalanxOutlineCorrect&STC (0.869415808)&InceptionTime (0.865979381)&WEASEL (0.855670103)\\ 
MiddlePhalanxTW&ROCKET (0.865979381)&ProximityForest (0.862542955)&ResNet (0.855670103)\\ 
MixedShapesRegularTrain&TS-CHIEF (0.981030928)&InceptionTime \& WEASEL (0.975257732)&\\ 
MixedShapesSmallTrain&ResNet (0.978969072)&HIVE-COTE v1.0 (0.976907216)&ROCKET (0.974845361)\\ 
MoteStrain&TS-CHIEF (0.96884984)&HIVE-COTE v1.0 (0.966185567)&WEASEL (0.956070288)\\ 
OliveOil&STC \& RISE \& TSF (1.0)&\\ 
OSULeaf&ROCKET \& ProximityForest (1.0)&TS-CHIEF \& S-BOSS (0.995867769)\\ 
PhalangesOutlinesCorrect&HIVE-COTE v1.0 (0.962340967)&ROCKET (0.958677686)&ResNet (0.956234097)\\ 
Phoneme&HIVE-COTE v1.0 \& ResNet (0.966666667)&Catch22 (0.883969466)\\ 
PigAirwayPressure&STC (0.995192308)&HIVE-COTE v1.0 \& ResNet (0.987603306)&\\ 
PigArtPressure&S-BOSS (1.0)&Over 3 methods (0.995192308)&\\ 
PigCVP&TS-CHIEF (0.985576923)&S-BOSS (0.980769231)&cBOSS \& BOSS (0.975961538)\\ 
Plane&Over 3 methods (1.0)&\\ 
ProximalPhalanxOutlineAgeGroup&ProximityForest (1.0)&ROCKET (0.988888889)&HIVE-COTE v1.0 (0.975961538)\\ 
ProximalPhalanxOutlineCorrect&HIVE-COTE v1.0 \& ResNet (1.0)&InceptionTime (0.93814433)\\ 
ProximalPhalanxTW&HIVE-COTE v1.0 \& Catch22 (1.0)&ResNet (0.922222222)\\ 
RefrigerationDevices&Catch22 (0.938888889)&HIVE-COTE v1.0 (0.887804878)&ROCKET \& ResNet (0.848780488)\\ 
Rock&STC (0.96)&WEASEL (0.94)&ResNet (0.927835052)\\ 
ScreenType&ROCKET (0.9)&Catch22 (0.865979381)&ProximityForest (0.86)\\ 
SemgHandGenderCh2&TS-CHIEF (0.968333333)&TSF (0.965)&STC (0.958333333)\\ 
SemgHandMovementCh2&ProximityForest (0.98)&ROCKET (0.95)&HIVE-COTE v1.0 (0.94)\\ 
SemgHandSubjectCh2&TSF (0.953333333)&TS-CHIEF (0.951111111)&STC (0.937777778)\\ 
ShapeletSim&Over 3 methods (1.0)&\\ 
ShapesAll&ROCKET (1.0)&InceptionTime (0.96)&TS-CHIEF (0.958333333)\\ 
SmallKitchenAppliances&HIVE-COTE v1.0 (0.968888889)&ROCKET (0.941666667)&ProximityForest (0.911666667)\\ 
SmoothSubspace&Over 3 methods (1.0)&\\ 
SonyAIBORobotSurface1&ProximityForest \& Catch22 (1.0)&ROCKET (0.993333333)\\ 
SonyAIBORobotSurface2&ROCKET (0.981697171)&InceptionTime (0.974816369)&ProximityForest (0.965058236)\\ 
StarLightCurves&HIVE-COTE v1.0 \& ResNet (1.0)&TS-CHIEF (0.98348713)\\ 
Strawberry&WEASEL (0.991891892)&Over 3 methods (0.989189189)&\\ 
SwedishLeaf&ROCKET \& ProximityForest (0.991891892)&ResNet (0.989506821)\\ 
Symbols&TS-CHIEF (0.987939698)&InceptionTime (0.985929648)&HIVE-COTE v1.0 (0.981787275)\\ 
SyntheticControl&Over 3 methods (1.0)&\\ 
ToeSegmentation1&ROCKET \& ProximityForest (1.0)&WEASEL \& S-BOSS \& cBOSS (0.986842105)\\ 
ToeSegmentation2&TS-CHIEF \& InceptionTime (0.992307692)&cBOSS \& BOSS (0.984615385)\\ 
Trace&Over 3 methods (1.0)&\\ 
TwoLeadECG&Over 3 methods (1.0)&\\ 
TwoPatterns&TS-CHIEF \& ROCKET \& InceptionTime (1.0)&\\ 
UMD&Over 3 methods (1.0)&\\ 
UWaveGestureLibraryAll&Over 3 methods (1.0)&\\ 
Wafer&STC \& WEASEL \& cBOSS (1.0)&\\ 
Wine&Over 3 methods (1.0)&\\ 
WordSynonyms&ROCKET \& ProximityForest (1.0)&TS-CHIEF (0.827586207)\\ 
Worms&HIVE-COTE v1.0 \& ResNet (1.0)&STC \& WEASEL (0.883116883)\\ 
WormsTwoClass&HIVE-COTE v1.0 \& ResNet (1.0)&Catch22 (0.999026606)\\ 
Yoga&cBOSS (0.937333333)&InceptionTime (0.933666667)&HIVE-COTE v1.0 (0.931)\\ 
\end{tabular}
}
\label{ Label *** }
\end{table*}






==> tables/rankByMethod.tex <==
\begin{table*}[!h]
\centering
\caption{ Legenda *** }
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccccccccccccccc}
&CNN&TS-CHIEF&HIVE-COTE v1.0&ROCKET&InceptionTime&STC&ResNet&ProximityForest&WEASEL&S-BOSS&cBOSS&BOSS&RISE&TSF&Catch22\\ 
\hline
First&6&35&32&26&31&21&25&23&20&20&20&18&12&14&11\\ 
Second&0&6&9&10&12&2&9&4&7&4&2&4&1&2&1\\ 
Third&1&7&5&12&5&6&11&4&5&4&3&3&0&1&5\\ 
\end{tabular}
}
\label{ Label *** }
\end{table*}



==> tables/shapiro.tex <==
\begin{table*}
\centering
\caption{Shapiro-Willis \textit{p}-values comparing all methods for the 6 selected UCR problems. Significant results~($p < 0.01$) are represented in \green{\underline{green}}.}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{c|cccccc}
&BME&Coffee&Earthquakes&Plane&SmoothSubspace&Trace\\ 
 \hline 
CNN&\green{\underline{0.0000}}&1.0000&\green{\underline{0.0000}}&1.0000&\green{\underline{0.0000}}&1.0000\\ 
TS-CHIEF&\green{\underline{0.0000}}&\green{\underline{0.0000}}&1.0000&1.0000&\green{\underline{0.0000}}&1.0000\\ 
HIVE-COTE v1.0&\green{\underline{0.0002}}&\green{\underline{0.0000}}&\green{\underline{0.0000}}&1.0000&\green{\underline{0.0131}}&1.0000\\ 
ROCKET&\green{\underline{0.0000}}&1.0000&\green{\underline{0.0000}}&1.0000&\green{\underline{0.0009}}&1.0000\\ 
InceptionTime&\green{\underline{0.0000}}&\green{\underline{0.0000}}&\green{\underline{0.0283}}&\green{\underline{0.0000}}&\green{\underline{0.0016}}&1.0000\\ 
STC&\green{\underline{0.0108}}&\green{\underline{0.0000}}&\green{\underline{0.0000}}&\green{\underline{0.0000}}&0.5589&1.0000\\ 
ResNet&\green{\underline{0.0000}}&\green{\underline{0.0000}}&0.5306&1.0000&\green{\underline{0.0001}}&1.0000\\ 
ProximityForest&\green{\underline{0.0000}}&\green{\underline{0.0000}}&\green{\underline{0.0038}}&1.0000&\green{\underline{0.0000}}&1.0000\\ 
WEASEL&\green{\underline{0.0001}}&\green{\underline{0.0000}}&\green{\underline{0.0000}}&\green{\underline{0.0000}}&0.5455&1.0000\\ 
S-BOSS&\green{\underline{0.0383}}&\green{\underline{0.0000}}&\green{\underline{0.0000}}&\green{\underline{0.0000}}&0.2508&1.0000\\ 
cBOSS&0.4336&\green{\underline{0.0000}}&\green{\underline{0.0000}}&1.0000&0.6805&1.0000\\ 
BOSS&\green{\underline{0.0010}}&\green{\underline{0.0000}}&\green{\underline{0.0000}}&\green{\underline{0.0000}}&0.3218&1.0000\\ 
RISE&\green{\underline{0.0217}}&\green{\underline{0.0000}}&1.0000&\green{\underline{0.0000}}&0.4091&\green{\underline{0.0018}}\\ 
TSF&\green{\underline{0.0041}}&\green{\underline{0.0000}}&\green{\underline{0.0000}}&\green{\underline{0.0000}}&\green{\underline{0.0068}}&\green{\underline{0.0000}}\\ 
Catch22&\green{\underline{0.0129}}&\green{\underline{0.0000}}&\green{\underline{0.0018}}&\green{\underline{0.0015}}&\green{\underline{0.0401}}&\green{\underline{0.0000}}\\ 
\end{tabular}
}
\label{table:shapiro}
\end{table*}

